The Compact Linear e$^+$e$^-$ Collider (CLIC)

The Compact Linear Collider (CLIC) is a TeV-scale high-luminosity linear e$^+$e$^-$ collider studied by the international CLIC and CLICdp collaborations. CLIC uses a two-beam acceleration scheme, in which normal-conducting high-gradient 12 GHz accelerating structures are powered via a high-current drive beam. CLIC is foreseen to be built and operated in stages. The initial 380 GeV stage, with a site length of 11 km, optimally combines the exploration of Higgs and top-quark physics, including a top threshold scan near 350 GeV. A higher-energy stage, still using the initial single drive-beam complex, can be optimised for any energy up to 2 TeV. Parameters are presented in detail for a 1.5 TeV stage, with a site length of 29 km. Since the 2018 ESPPU reporting, significant effort was invested in CLIC accelerator optimisation, technology developments and system tests, including collaboration with new-generation light sources and free-electron lasers. CLIC implementation aspects at CERN have covered detailed studies of civil engineering, electrical networks, cooling and ventilation, scheduling, and costing. The CLIC baseline at 380 GeV is now 100 Hz operation, with a luminosity of 4.5$\times 10^{34}$ cm$^{-2}$s$^{-1}$ and a power consumption of 166 MW. Compared to the 2018 design, this gives three times higher luminosity-per-power. The new baseline has two beam-delivery systems, allowing for two detectors operating in parallel. The cost estimate of the 380 GeV baseline is approximately 7.2 billion CHF. The construction of the first CLIC energy stage could start as early as ~2034/35 with first beams following a decade later. This report summarises the CLIC project, its implementation and running scenarios, with emphasis on new developments and recent progress. It concludes with an update on the CLIC detector studies and on the physics potential in light of the improved accelerator performance.

==> authors/authors_modified.tex <==
{\footnotesize
\begin{multicols}{2}
\begin{center}{
T.K.~Charles, % added, from Monash Univ.
P.J.~Giansiracusa,
T.G.~Lucas,
R.P.~Rassool,
M.~Volpi$^{1}$\\% added
}\textbf{University of Melbourne, Melbourne, Australia}
\end{center}
\vspace{-0.5cm}

\begin{center}{
C.~Balazs\\ %CLICdp
}\textbf{Monash University, Melbourne, Australia}
\end{center}
\vspace{-0.5cm}

\begin{center}{
K.~Afanaciev, % CLICdp
V.~Makarenko\\%CLICdp 
}\textbf{Belarusian State University, Minsk, Belarus}
\end{center}
\vspace{-0.5cm}

\begin{center}{
A.~Patapenka, 
I.~Zhuk\\
}\textbf{Joint Institute for Power and Nuclear Research - Sosny, Minsk, Belarus}
\end{center}
\vspace{-0.5cm}

\begin{center}{
C.~Collette\\
}\textbf{Universit\'e libre de Bruxelles, Brussels, Belgium}
\end{center}
\vspace{-0.5cm}

\begin{center}{
M.J.~Boland\\   % added
}\textbf{University of Saskatchewan, Saskatoon, Canada}
\end{center}
\vspace{-0.5cm}

\begin{center}{
A.C.~Abusleme~Hoffman,
M.A.~Diaz,
F.~Garay\\
}\textbf{Pontificia Universidad Cat\'{o}lica de Chile, Santiago, Chile}
\end{center}
\vspace{-0.5cm}

\begin{center}{
Y.~Chi,
X.~He,
G.~Pei,
S.~Pei,
G.~Shu,
X.~Wang,
J.~Zhang,
F.~Zhao,
Z.~Zhou\\
}\textbf{Institute of High Energy Physics, Beijing, China}
\end{center}
\vspace{-0.5cm}

\begin{center}{
H.~Chen,
Y.~Gao,
W.~Huang,
Y.P.~Kuang,
B.~Li,
Y.~Li,
X.~Meng, % added
J.~Shao,
J.~Shi,
C.~Tang,
P.~Wang, % added
X.~Wu,
H.~Zha\\ % added, was at CERN
}\textbf{Tsinghua University, Beijing, China}
\end{center}
\vspace{-0.5cm}

\begin{center}{
L.~Ma,
Y.~Han\\
}\textbf{Shandong University, Jinan, China}
\end{center}
\vspace{-0.5cm}

\begin{center}{
W.~Fang,
Q.~Gu, 
D.~Huang, 
X.~Huang, 
J.~Tan, 
Z.~Wang, 
Z.~Zhao\\
}\textbf{Shanghai Institute of Applied Physics, Chinese Academy of Sciences, Shanghai, China}
\end{center}
\vspace{-0.5cm}

\begin{center}{
U.I.~Uggerh{\o}j,
T.N.~Wistisen\\
}\textbf{Aarhus University, Aarhus, Denmark}
\end{center}
\vspace{-0.5cm}

\begin{center}{
A.~Aabloo,
R.~Aare, % added
K.~Kuppart,
S.~Vigonski,
V.~Zadin\\
}\textbf{University of Tartu, Tartu, Estonia}
\end{center}
\vspace{-0.5cm}

\begin{center}{
M.~Aicheler,
E.~Baibuz,
E.~Br\"{u}cken,
F.~Djurabekova$^{2}$,
P.~Eerola$^{2}$,
F.~Garcia,
E.~Haeggstr\"{o}m$^{2}$,
K.~Huitu$^{2}$,
V.~Jansson$^{2}$,
I.~Kassamakov$^{2}$,
J.~Kimari$^{2}$,  % added
A.~Kyritsakis,
S.~Lehti,
A.~ Meril\"{a}inen$^{2}$,
R.~Montonen$^{2}$,
K.~Nordlund$^{2}$,
K.~\"{O}sterberg$^{2}$,
A.~Saressalo,  % added
J.~V\"{a}in\"{o}l\"{a},
M.~Veske\\
}\textbf{Helsinki Institute of Physics, University of Helsinki, Helsinki, Finland}
\end{center}
\vspace{-0.5cm}

\begin{center}{
W.~Farabolini,
A.~Mollard,
F.~Peauger$^{3}$, % RR: added now at CERN
J.~Plouin\\
}\textbf{CEA, Gif-sur-Yvette, France}
\end{center}
\vspace{-0.5cm}

\begin{center}{
P.~Bambade,
I.~Chaikovska,
R.~Chehab,
N.~Delerue, % added
M.~Davier,
A.~Faus-Golfe, % added
A.~Irles, % added
W.~Kaabi,
F.~LeDiberder,
R.~P\"{o}schl,
D.~Zerwas\\
}\textbf{Laboratoire de l'Acc\'{e}l\'{e}rateur Lin\'{e}aire, Universit\'{e} de Paris-Sud XI, IN2P3/CNRS, Orsay, France}
\end{center}
\vspace{-0.5cm}

\begin{center}{
B.~Aimard,
G.~Balik,
J.-J.~Blaising, % CLICdp
L.~Brunetti,
M.~Chefdeville, % CLICdp - not requested by CLICdp interface, leave "just in case"
A.~Dominjon, % added
C.~Drancourt,
N.~Geoffroy,
J.~Jacquemier,
A.~Jeremie,
Y.~Karyotakis,
J.M.~Nappa,
M.~Serluca, % added
S.~Vilalte,
G.~Vouters\\
}\textbf{LAPP, Universit\'{e} de Savoie, IN2P3/CNRS, Annecy, France}
\end{center}
\vspace{-0.5cm}

\begin{center}{
A.~Bernhard, % corrected spelling (h was missing)
E.~Br\"{u}ndermann, %%added
S.~Casalbuoni, % added
S.~Hillenbrand, % added
J.~Gethmann, % added
A.~Grau, % added
E.~Huttel, % added
A.-S.~M\"{u}ller, %%added
P.~Peiffer$^{4}$,  % added
I.~Peri\'{c},
D. Saez de Jauregui\\
}\textbf{Karlsruhe Institute of Technology (KIT), Karlsruhe, Germany} % corrected spelling
\end{center}
\vspace{-0.5cm}

\begin{center}{
L.~Emberger,
C.~Graf,
F.~Simon,
M.~Szalay,
N.~van~der~Kolk$^{5}$\\
}\textbf{Max-Planck-Institut f\"{u}r Physik, Munich, Germany}
\end{center}
\vspace{-0.5cm}

\begin{center}{
S.~Brass,
W.~Kilian\\
}\textbf{Department of Physics, University of Siegen, Siegen, Germany}
\end{center}
\vspace{-0.5cm}


\begin{center}{
T.~Alexopoulos,
T.~Apostolopoulos$^{6}$,  % added
E.N.~Gazis,
N.~Gazis,
V.~Kostopoulos$^{7}$,
S.~Kourkoulis\\
}\textbf{National Technical University of Athens, Athens, Greece}
\end{center}
\vspace{-0.5cm}


\begin{center}{
B.~Heilig\\
}\textbf{Department of Basic Geophysical Research, Mining and Geological Survey of Hungary, Tihany, Hungary}
\end{center}
\vspace{-0.5cm}


\begin{center}{
J.~Lichtenberger\\
}\textbf{Space Research Laboratory, E\"otv\"os Lor\'and University, Budapest, Hungary}
\end{center}
\vspace{-0.5cm}



\begin{center}{
P.~Shrivastava\\
}\textbf{Raja Ramanna Centre for Advanced Technology, Department of Atomic Energy, Indore, India}
\end{center}
\vspace{-0.5cm}

\begin{center}{
M.K.~Dayyani,
H.~Ghasem$^{1}$,
S.S.~Hajari,
H.~Shaker$^{1}$\\
}\textbf{The School of Particles and Accelerators, Institute for Research in Fundamental Sciences, Tehran, Iran}
\end{center}
\vspace{-0.5cm}

\begin{center}{
Y.~Ashkenazy,
I.~Popov, % added
E.~Engelberg, % added
A. Yashar\\ % added
}\textbf{Racah Institute of Physics, Hebrew University of Jerusalem, Jerusalem, Israel}
\end{center}
\vspace{-0.5cm}

\begin{center}{
H.~Abramowicz,
Y.~Benhammou,
O.~Borysov,
M.~Borysova,
A.~Levy,
I.~Levy\\
}\textbf{Raymond \& Beverly Sackler School of Physics  \& Astronomy, Tel Aviv University, Tel Aviv, Israel}
\end{center}
\vspace{-0.5cm}

\begin{center}{
D.~Alesini,
M.~Bellaveglia,
B.~Buonomo,
A.~Cardelli,
M.~Diomede,
M.~Ferrario,
A.~Gallo,
A.~Ghigo,
A.~Giribono,
L.~Piersanti,
A.~Stella,
C.~Vaccarezza\\
}\textbf{INFN e Laboratori Nazionali di Frascati, Frascati, Italy}
\end{center}
\vspace{-0.5cm}

\begin{center}{
J.~de~Blas\\
}\textbf{Universit\`{a} di Padova and INFN, Padova, Italy}
\end{center}
\vspace{-0.5cm}

\begin{center}{
R.~Franceschini\\
}\textbf{Universit\`{a} degli Studi Roma Tre and INFN, Roma, Italy}
\end{center}
\vspace{-0.5cm}

\begin{center}{
G.~D'Auria, 
S.~Di Mitri\\
}\textbf{Elettra Sincrotrone Trieste, Trieste, Italy}
\end{center}
\vspace{-0.5cm}

\begin{center}{
T.~Abe, 
A.~Aryshev,
M.~Fukuda, % added
K.~Furukawa, % added 
H.~Hayano, % added
Y.~Higashi, % added
T.~Higo,
K.~Kubo, % added
S.~Kuroda, % adde
S.~Matsumoto, 
S.~Michizono, % added
T.~Naito, % added
T.~Okugi, % added
T.~Shidara, 
T.~Tauchi, 
N.~Terunuma, % added
J.~Urakawa, 
A.~Yamamoto$^{1}$\\
}\textbf{High Energy Accelerator Research Organization, KEK, Tsukuba, Japan}
\end{center}
\vspace{-0.5cm}

\begin{center}{
R.~Raboanary\\
}\textbf{University of Antananarivo, Antananarivo, Madagascar}
\end{center}
\vspace{-0.5cm}

\begin{center}{
O.J.~Luiten,
X.F.D.~Stragier\\
}\textbf{Eindhoven University of Technology, Eindhoven, Netherlands}
\end{center}
\vspace{-0.5cm}


\begin{center}{
R.~Hart,
H.~van der Graaf\\
}\textbf{Nikhef, Amsterdam, Netherlands}
\end{center}
\vspace{-0.5cm}

\begin{center}{
G.~Eigen\\
}\textbf{Department of Physics and Technology, University of Bergen, Bergen, Norway}
\end{center}
\vspace{-0.5cm}

\begin{center}{
E.~Adli$^{1}$,
C.A.~Lindstr{\o}m, % added
R.~Lillest\o{}l,
L.~Malina$^1$,
J.~Pfingstner,
K.N.~Sjobak$^1$\\
}\textbf{University of Oslo, Oslo, Norway}
\end{center}
\vspace{-0.5cm}

\begin{center}{
A.~Ahmad, % added
H.~Hoorani,
W.A.~Khan\\ % added
}\textbf{National Centre for Physics, Islamabad, Pakistan}
\end{center}
\vspace{-0.5cm}

\begin{center}{
S.~Bugiel,
R.~Bugiel,
M.~Firlej,
T.A.~Fiutowski,
M.~Idzik,
J.~Moro\'{n},
K.P.~\'{S}wientek\\
}\textbf{AGH University of Science and Technology, Krakow, Poland}
\end{center}
\vspace{-0.5cm}

\begin{center}{
P.~Br\"{u}ckman~de~Renstrom, % added
B.~Krupa,
M.~Kucharczyk,
T.~Lesiak,
B.~Pawlik,
P.~Sopicki,
B.~Turbiarz,
T.~Wojto\'{n},
L.K.~Zawiejski\\
}\textbf{Institute of Nuclear Physics, Polish Academy of Sciences, Krakow, Poland}
\end{center}
\vspace{-0.5cm}

\begin{center}{
J.~Kalinowski,
K.~Nowak,
A.F.~\.{Z}arnecki\\
}\textbf{Faculty of Physics, University of Warsaw, Warsaw, Poland}
\end{center}
\vspace{-0.5cm}

\begin{center}{
E.~Firu,
V.~Ghenescu,
A.T.~Neagu,
T.~Preda,
I. S. Zgura\\
}\textbf{Institute of Space Science, Bucharest, Romania}
\end{center}
\vspace{-0.5cm}

\begin{center}{
A.~Aloev,
N.~Azaryan,
I.~Boyko, %CLICdp
J.~Budagov,
M.~Chizhov,
M.~Filippova,
V.~Glagolev,
A.~Gongadze,
S.~Grigoryan,
D.~Gudkov,
V.~Karjavine,
M.~Lyablin,
Yu.~Nefedov, %CLICdp
A.~Olyunin$^{1}$,
A.~Rymbekova, %CLICdp
A.~Samochkine,
A.~Sapronov, % also CLICdp
G.~Shelkov, %CLICdp
G.~Shirkov,
V.~Soldatov,
E.~Solodko$^{1}$,
G.~Trubnikov,
I.~Tyapkin,
V.~Uzhinsky,
A.~Vorozhtov,
A.~Zhemchugov\\ % CLICdp
}\textbf{Joint Institute for Nuclear Research, Dubna, Russia} %this name received for CLICdp
\end{center}
\vspace{-0.5cm}

\begin{center}{
E.~Levichev,
N.~Mezentsev,
P.~Piminov,
D.~Shatilov,
P.~Vobly,
K.~Zolotarev\\
}\textbf{Budker Institute of Nuclear Physics, Novosibirsk, Russia}
\end{center}
\vspace{-0.5cm}


\begin{center}{
I.~Bo\v{z}ovi\'{c} Jelisav\v{c}i\'{c},
G.~Ka\v{c}arevi\'{c},
G.~Milutinovi\'{c} Dumbelovi\'{c},
M.~Pandurovi\'{c},
M.~Radulovi\'{c},
J. ~Stevanovi\'{c},
N.~Vukasinovi\'{c}\\
}\textbf{Vin\v{c}a Institute of Nuclear Sciences, University of Belgrade, Belgrade, Serbia}
\end{center}
\vspace{-0.5cm}


\begin{center}{
D.-H.~Lee\\
}\textbf{School of Space Research, Kyung Hee University, Yongin, Gyeonggi, South Korea}
\end{center}
\vspace{-0.5cm}

\begin{center}{
N.~Ayala, % added
G.~Benedetti, % added
T.~Guenzel, % added
U.~Iriso,
Z.~Marti, % added
F.~Perez,
M.~Pont\\
}\textbf{CELLS-ALBA, Barcelona, Spain}
\end{center}
\vspace{-0.5cm}


\begin{center}{
J.~Trenado\\
}\textbf{University of Barcelona, Barcelona, Spain}
\end{center}
\vspace{-0.5cm}

\begin{center}{
A.~Ruiz-Jimeno,
I.~Vila\\
}\textbf{IFCA, CSIC-Universidad de Cantabria, Santander, Spain}
\end{center}
\vspace{-0.5cm}

\begin{center}{
J.~Calero, 
M.~Dominguez, % added
L.~Garcia-Tabares,
D.~Gavela,
D.~Lopez,
F.~Toral\\
}\textbf{Centro de Investigaciones Energ\'{e}ticas, Medioambientales y Tecnol\'{o}gicas (CIEMAT), Madrid, Spain}
\end{center}
\vspace{-0.5cm}

\begin{center}{

C.~Blanch Gutierrez,
M.~Boronat,
D.~Esperante$^{1}$,
E.~Fullana,
J.~Fuster,
 I.~Garc\'{\i}a, % removed  -- reinserted for CLICdp
B.~Gimeno, % added
P.~Gomis Lopez, % added
D.~Gonz\'{a}lez, % added
M.~Perell\'{o}, % added
E.~Ros,
M.A.~Villarejo, % added
A.~Vnuchenko, % added
M.~Vos\\
}\textbf{Instituto de F\'{\i}sica Corpuscular (CSIC-UV), Valencia, Spain}
\end{center}
\vspace{-0.5cm}

\begin{center}{
R.~Brenner, 
Ch.~Borgmann,
T.~Ekel\"{o}f, 
M.~Jacewicz,  
M.~Olveg{\aa}rd, 
R.~Ruber, 
V.~Ziemann\\
}\textbf{Uppsala University, Uppsala, Sweden}
\end{center}
\vspace{-0.5cm}

\begin{center}{
D.~Aguglia,
J.~Alabau Gonzalvo,
M.~Alcaide Leon, % added
N.~Alipour~Tehrani, 
M.~Anastasopoulos, %RC
A.~Andersson,
F.~Andrianala$^{8}$,
F.~Antoniou,
A.~Apyan, %RC
D.~Arominski$^{9}$,
K.~Artoos,
S.~Assly,
S.~Atieh,
C.~Baccigalupi, %RC
R.~Ballabriga~Sune,
D.~Banon~Caballero,
M.J.~Barnes,
J.~Barranco~Garcia,
A.~Bartalesi, %RC
J.~Bauche,
C.~Bayar, % added, PhD student from Ankara
C.~Belver-Aguilar,
A.~Benot Morell$^{10}$,
M.~Bernardini, % added %SS
D.R.~Bett,
S.~Bettoni$^{11}$, %RC   
M.~Bettencourt, %RC 
B.~Bielawski, %RC
O.~Blanco Garcia,
N.~Blaskovic Kraljevic, % added
B.~Bolzon$^{12}$,  
X.A.~Bonnin,
D.~Bozzini,
E.~Branger, %RC
E.~Brondolin,
O.~Brunner,
M.~Buckland$^{13}$,   
H.~Bursali, %RC
H.~Burkhardt,
D.~Caiazza, %RC
S.~Calatroni, 
M.~Campbell,
N.~Catalan~Lasheras,
B.~Cassany,
E.~Castro, 
R.H.~Cavaleiro Soares, %RC
M.~Cerqueira~Bastos,
A.~Cherif,
E.~Chevallay,
V.~Cilento$^{14}$,  
R.~Corsini, 
R.~Costa$^{15}$,  
B.~Cure, 
S.~Curt,
A.~Dal Gobbo, %RC
D.~Dannheim,
E.~Daskalaki, %RC
L.~Deacon, %RC
A.~Degiovanni, %RC
G.~De~Michele,
L.~De~Oliveira,
V.~Del~Pozo~Romano,
J.P.~Delahaye,
D.~Delikaris,
P.G.~Dias~de~Almeida$^{16}$,     
T.~Dobers,
S.~Doebert,
I.~Doytchinov, %RC
M.~Draper,
F.~Duarte~Ramos,
M.~Duquenne, %RC
N.~Egidos~Plaja,
K.~Elsener,
J.~Esberg,
M.~Esposito,
L.~Evans,
V.~Fedosseev,
P.~Ferracin,
A.~Fiergolski,
K.~Foraz,
A.~Fowler,
F.~Friebel,
J-F.~Fuchs,
A.~Gaddi,
D.~Gamba, % added, was at Oxford
L.~Garcia~Fajardo$^{17}$,    
H.~Garcia~Morales,
C.~Garion,
M.~Gasior, % added
L.~Gatignon,
J-C.~Gayde,
A.~Gerbershagen, %RC
H.~Gerwig,
G.~Giambelli, %RC
A.~Gilardi, %RC
A.N.~Goldblatt,
S.~Gonzalez~Anton, % added
C.~Grefe$^{18}$,    
A.~Grudiev,
H.~Guerin, %RC
F.G.~Guillot-Vignot,
M.L.~Gutt-Mostowy,
M.~Hein Lutz, %RC
C.~Hessler,
J.K.~Holma,
E.B.~Holzer,
M.~Hourican,
D.~Hynds$^{19}$, 
E.~Ikarios,  %RC
Y.~Inntjore~Levinsen,
S.~Janssens, %RC
A.~Jeff, % added    
E.~Jensen,
M.~Jonker,
S.W.~Kamugasa, %RC
M.~Kastriotou,
J.M.K.~Kemppinen,
V.~Khan, %RC
R.B.~Kieffer,
W.~Klempt,
N.~Kokkinis,
I.~Kossyvakis, %RC
Z.~Kostka, %RC
A.~Korsback,
E.~Koukovini~Platia,
J.W.~Kovermann,
C-I.~Kozsar,
I.~Kremastiotis$^{20}$,
J.~Kr\"{o}ger$^{21}$,
S.~Kulis,
A.~Latina,
F.~Leaux,
P.~Lebrun, %
T.~Lefevre,
E.~Leogrande,
L.~Linssen,
X.~Liu, % added
X.~Llopart~Cudie,
S.~Magnoni,  %RC
C.~Maidana, %RC
A.A.~Maier,
H.~Mainaud~Durand,
S.~Mallows, %RC
E.~Manosperti,
C.~Marelli, %RC
E.~Marin~Lacoma,
S.~Marsh, % added
R.~Martin,
I.~Martini, %RC
M.~Martyanov, %RC
S.~Mazzoni,
G.~Mcmonagle,
L.M.~Mether,
C.~Meynier, %RC
M.~Modena,
A.~Moilanen, %RC
R.~Mondello, %RC
P.B.~Moniz Cabral,
N.~Mouriz Irazabal, %RC
M.~Munker,
T.~Muranaka,
J.~Nadenau, % added
J.G.~Navarro, % added
J.L.~Navarro Quirante, %RC
E.~Nebo~ Del~Busto,
N.~Nikiforou$^{22}$,
P.~Ninin,
M.~Nonis,
D.~Nisbet,
F.X.~Nuiry,
A.~N\"{u}rnberg$^{23}$,
J.~\"{O}gren, % added, was at Uppsala
J.~Osborne,
A.C.~Ouniche, %RC
R.~Pan$^{24}$, % added   
S.~Papadopoulou,
Y.~Papaphilippou,
G.~Paraskaki, %RC
A.~Pastushenko$^{10}$, % added    
A.~Passarelli,
M.~Patecki,
L.~Pazdera,
D.~Pellegrini,
K.~Pepitone,
E.~Perez~Codina,
A.~Perez~Fontenla,
T.H.B.~Persson,
M.~Petri\v{c}$^{25}$,
S.~Pitman, % added      
F.~Pitters$^{26}$,
S.~Pittet,
F.~Plassard,
D.~Popescu, %RC 
T.~Quast$^{27}$,
R.~Rajamak,
S.~Redford$^{11}$,
L.~Remandet, %RC
Y.~Renier$^{24}$,
S.F.~Rey,
O.~Rey~Orozco, %added
G.~Riddone,
E.~Rodriguez~Castro,
P.~Roloff,    %
C.~Rossi,
F.~Rossi, %RC
V.~Rude,
I.~Ruehl, % added
G.~Rumolo,
A.~Sailer,
J.~Sandomierski, %RC
E.~Santin,
C.~Sanz, %RC
J.~Sauza Bedolla, % added
U.~Schnoor,
H.~Schmickler,
D.~Schulte,
E.~Senes, %RC
C.~Serpico,
G.~Severino, %RC
N.~Shipman,
E.~Sicking,
R.~Simoniello$^{28}$,
P.K.~Skowronski,
P.~Sobrino~Mompean,
L.~Soby,
P.~Sollander,
A.~Solodko, % added, was at Dubna, Russia
M.P.~Sosin,
S.~Spannagel,
S.~Sroka,
S.~Stapnes,
G.~Sterbini,
G.~Stern, %RC
R.~Str\"{o}m,
M.J.~Stuart,
I.~Syratchev,
K.~Szypula, % added
F.~Tecker,
P.A.~Thonet,
P.~Thrane, %RC
L.~Timeo,
M.~Tiirakari, % added
R.~Tomas~Garcia,
C.I.~Tomoiaga, %RC
P.~Valerio$^{29}$,
T.~Va\v{n}\'{a}t,
A.L.~Vamvakas,
J.~Van~Hoorne,  %RC
O.~Viazlo,
M.~Vicente~Barreto~Pinto$^{30}$,
N.~Vitoratou, %RC
V.~Vlachakis, %RC
M.A.~Weber,
R.~Wegner,
M.~Wendt,
M.~Widorski,
O.E.~Williams, % added
M.~Williams$^{31}$,
B.~Woolley,
W.~Wuensch,
A.~Wulzer,
J.~Uythoven,
A.~Xydou, %RC
R.~Yang,
A.~Zelios, %RC
Y.~Zhao$^{32}$, % added    
P.~Zisopoulos\\
}\textbf{CERN, Geneva, Switzerland}
\end{center}
\vspace{-0.5cm}



\begin{center}{
M.~Benoit,
D~M~S~Sultan\\
}\textbf{D\'{e}partement de Physique Nucl\'{e}aire et Corpusculaire (DPNC), Universit\'{e} de Gen\`{e}ve, Gen\`{e}ve, Switzerland}
\end{center}
\vspace{-0.5cm}

\begin{center}{
F.~Riva$^{1}$\\
}\textbf{D\'{e}partement de Physique Th\'{e}orique, Universit\'{e} de Gen\`{e}ve, Gen\`{e}ve, Switzerland}
\end{center}
\vspace{-0.5cm}

\begin{center}{
M.~Bopp,
H.H.~Braun,
P.~Craievich, %added
M.~Dehler,
T.~Garvey,
M.~Pedrozzi, % added
J.Y.~Raguin,
L.~Rivkin$^{33}$,
R.~Zennaro\\
}\textbf{Paul Scherrer Institut, Villigen, Switzerland}
\end{center}
\vspace{-0.5cm}

\begin{center}{
S.~Guillaume,  % added
M.~Rothacher\\  % added
}\textbf{ETH Zurich, Institute of Geodesy and Photogrammetry, Zurich, Switzerland}
\end{center}
\vspace{-0.5cm}

\begin{center}{
A.~Aksoy,
Z.~Nergiz$^{34}$,
\"{O}.~Yavas\\
}\textbf{Ankara University, Ankara, Turkey}
\end{center}
\vspace{-0.5cm}

\begin{center}{
H.~Denizli,
U.~Keskin, 
K.~Y.~Oyulmaz,
A.~Senol\\
}\textbf{Department of Physics, Abant \.{I}zzet Baysal University, Bolu, Turkey}
\end{center}
\vspace{-0.5cm}

\begin{center}{
A.K.~Ciftci\\
}\textbf{Izmir University of Economics, Izmir, Turkey}
\end{center}
\vspace{-0.5cm}

\begin{center}{
V.~Baturin,
O.~Karpenko, % added
R.~Kholodov,
O.~Lebed, % added
S.~Lebedynskyi,
S.~Mordyk,
I.~Musienko, %added
Ia.~Profatilova, % $^{1}$, updated
V.~Storizhko\\
}\textbf{Institute of Applied Physics, National Academy of Sciences of Ukraine, Sumy, Ukraine}
\end{center}
\vspace{-0.5cm}

\begin{center}{
R.R.~Bosley,
T.~Price,
M.F.~Watson,
N.K.~Watson,
A.G.~Winter\\
}\textbf{University of Birmingham, Birmingham, United Kingdom}
\end{center}
 
\begin{center}{
J.~Goldstein\\
}\textbf{University of Bristol, Bristol, United Kingdom}
\end{center}
\vspace{-0.5cm}

\begin{center}{
S.~Green,
J.S.~Marshall$^{35}$,
M.A.~Thomson,
B.~Xu,
T.~You$^{36}$\\
}\textbf{Cavendish Laboratory, University of Cambridge, Cambridge, United Kingdom}
\end{center}
\vspace{-0.5cm}

\begin{center}{
W.A.~Gillespie\\
}\textbf{University of Dundee, Dundee, United Kingdom}
\end{center}
\vspace{-0.5cm}

\begin{center}{
M.~Spannowsky\\
}\textbf{Department of Physics, Durham University, Durham, United Kingdom}
\end{center}
\vspace{-0.5cm}

\begin{center}{
C.~Beggan\\
}\textbf{British Geological Survey, Edinburgh, United Kingdom}
\end{center}
\vspace{-0.5cm}


\begin{center}{
V.~Martin,
Y.~Zhang\\
}\textbf{University of Edinburgh, Edinburgh, United Kingdom}
\end{center}
\vspace{-0.5cm}



\begin{center}{
D.~Protopopescu,
A.~Robson$^{1}$\\
}\textbf{University of Glasgow, Glasgow, United Kingdom}
\end{center}
\vspace{-0.5cm}


\begin{center}{
R.J.~Apsimon$^{37}$,
I.~Bailey$^{38}$,
G.C.~Burt$^{37}$,
A.C.~Dexter$^{37}$,
A.V.~Edwards$^{37}$, % added
V.~Hill$^{37}$, % added
S.~Jamison, % added %RC-2
W.L.~Millar$^{37}$, % added
K.~Papke$^{37}$\\  % added
}\textbf{Lancaster University, Lancaster, United Kingdom}
\end{center}
\vspace{-0.5cm}

\begin{center}{
G.~Casse, 
J.~Vossebeld\\
}\textbf{University of Liverpool, Liverpool, United Kingdom}
\end{center}
\vspace{-0.5cm}

\begin{center}{
T.~Aumeyr, % added
M.~Bergamaschi$^{1}$, % added %RC-2
L.~Bobb$^{38}$, % added
A.~Bosco, 
S.~Boogert, % from London 2
G.~Boorman, % from London 2
F.~Cullinan, % added
S.~Gibson, % from London 2
P.~Karataev,
K.~Kruchinin, % removed then added
K.~Lekomtsev, 
A.~Lyapin, % from London 2
L.~Nevay, 
W.~Shields, % from London 2
J.~Snuverink, % removed then added
J.~Towler, % added
E.~Yamakawa\\ % removed then added
}\textbf{The John Adams Institute for Accelerator Science, Royal Holloway, University of London, Egham, United Kingdom}
\end{center}
\vspace{-0.5cm}

\begin{center}{
V.~Boisvert,
S.~West\\
}\textbf{Royal Holloway, University of London, Egham, United Kingdom}
\end{center}
\vspace{-0.5cm}

\begin{center}{
R.~Jones,
N.~Joshi\\
}\textbf{University of Manchester, Manchester, United Kingdom}
\end{center}
\vspace{-0.5cm}

\begin{center}{

D.~Bett, % added
R.M.~Bodenstein$^{1}$, % updated, also at CERN
T.~Bromwich,
P.N.~Burrows$^{1}$, % updated, also at CERN
G.B.~Christian$^{38}$, % updated, now at Diamond
C.~Gohil$^{1}$, % added
P.~Korysko$^{1}$, % added
J.~Paszkiewicz$^{1}$, % added
C.~Perry,
R.~Ramjiawan, % added
J.~Roberts\\ % updated, removed also at CERN
}\textbf{John Adams Institute, Department of Physics, University of Oxford, Oxford, United Kingdom}
\end{center}
\vspace{-0.5cm}

\begin{center}{
T.~Coates,
F.~Salvatore\\
}\textbf{University of Sussex, Brighton, United Kingdom}
\end{center}
\vspace{-0.5cm}

\begin{center}{
A.~Bainbridge$^{37}$, % added
J.A.~Clarke$^{37}$,
N.~Krumpa,   %$^{38}$,						% added
B.J.A.~Shepherd$^{37}$,
D.~Walsh$^{3}$\\
}\textbf{STFC Daresbury Laboratory, Warrington, United Kingdom}
\end{center}
\vspace{-0.5cm}

\begin{center}{
S.~Chekanov, %added in CLICdp
M.~Demarteau, % CLICdp
W.~Gai, % added (accelerator)
W.~Liu, % added (accelerator)
J.~Metcalfe, % added in CLICdp
J.~Power, % added (accelerator)
J.~Repond, % CLICdp
H.~Weerts, % CLICdp
L.~Xia,     % CLICdp
J.~Zhang\\ % added in CLICdp
}\textbf{Argonne National Laboratory, Argonne, USA}
\end{center}
\vspace{-0.5cm}

\begin{center}{
J.~Zupan\\
}\textbf{Department of Physics, University of Cincinnati, Cincinnati, OH, USA}
\end{center}
\vspace{-0.5cm}

\begin{center}{
J.D.~Wells,
Z.~Zhang\\
}\textbf{Physics Department, University of Michigan, Ann Arbor, MI, USA}
\end{center}
\vspace{-0.5cm}

\begin{center}{
C.~Adolphsen, 
T.~Barklow, 
V.~Dolgashev, % added
M.~Franzi, % added
N.~Graf, 
J.~Hewett, 
M.~Kemp, % added
O.~Kononenko, %added  %%%%%%%%%%%% check for double counting %%%%%%%%%%%%
T.~Markiewicz, 
K.~Moffeit, 
J.~Neilson, % added
Y.~Nosochkov,
M.~Oriunno, 
N.~Phinney, 
T.~Rizzo, 
S.~Tantawi, 
J.~Wang, 
B.~Weatherford, % added
G.~White, 
M.~Woodley\\
}\textbf{SLAC National Accelerator Laboratory, Menlo Park, USA}
\end{center}
\vspace{-0.5cm}

\begin{flushleft}{
{$^{1}$}Also at CERN, Geneva, Switzerland\\
{$^{2}$}Also at Department of Physics, University of Helsinki, Helsinki, Finland\\
{$^{3}$}Now at CERN, Geneva, Switzerland\\
{$^{4}$}Now at Johannes-Gutenberg University, Mainz, Germany\\
{$^{5}$}Now at Nikhef / Utrecht University, Amsterdam / Utrecht, The Netherlands\\
{$^{6}$}Also at Department of Informatics, Athens University of Business and Economics, Athens, Greece \\
{$^{7}$}Also at University of Patras, Patras, Greece\\
{$^{8}$}Also at University of Antananarivo, Antananarivo, Madagascar\\
{$^{9}$}Also at Warsaw University of Technology, Warsaw, Poland\\
{$^{10}$}Also at IFIC, Valencia, Spain\\
{$^{11}$}Now at Paul Scherrer Institute, Villigen, Switzerland\\
{$^{12}$}Now at CEA, Gif-sur-Yvette, France\\   
{$^{13}$}Also at University of Liverpool, United Kingdom\\
{$^{14}$}Also at LAL, Orsay, France\\
{$^{15}$}Also at Uppsala University, Uppsala, Sweden\\ 
{$^{16}$}Also at IFCA, CSIC-Universidad de Cantabria, Santander, Spain\\
{$^{17}$}Now at LBNL, Berkeley CA, USA\\
{$^{18}$}Now at University of Bonn, Bonn, Germany\\
{$^{19}$}Now at Nikhef, Amsterdam, The Netherlands\\
{$^{20}$}Also at KIT, Karlsruhe, Germany\\
{$^{21}$}Also at Ruprecht-Karls-Universit\"{a}t Heidelberg, Germany\\
{$^{22}$}Now at University of Texas, Austin, USA\\
{$^{23}$}Now at Karlsruhe Institute of Technology, Karlsruhe, Germany\\
{$^{24}$}Now at DESY, Zeuthen, Germany\\
{$^{25}$}Also at J.\ Stefan Institute, Ljubljana, Slovenia\\
{$^{26}$}Also at Vienna University of Technology, Vienna, Austria\\
{$^{27}$}Also at RWTH Aachen University, Aachen, Germany\\
{$^{28}$}Now at Johannes Gutenberg Universit\"{a}t, Mainz, Germany\\
{$^{29}$}Now at D\'{e}partement de Physique Nucl\'{e}aire et Corpusculaire (DPNC), Universit\'{e} de Gen\`{e}ve, Geneva, Switzerland\\
{$^{30}$}Also at D\'{e}partement de Physique Nucl\'{e}aire et Corpusculaire (DPNC), Universit\'{e} de Gen\`{e}ve, Geneva, Switzerland\\
{$^{31}$}Also at University of Glasgow, Glasgow, United Kingdom\\
{$^{32}$}Also at Shandong University, Jinan, China\\
{$^{33}$}Also at EPFL, Lausanne, Switzerland\\
{$^{34}$}Also at Omer Halis Demir University, Nigde, Turkey\\
{$^{35}$}Now at University of Warwick, Coventry, United Kingdom\\
{$^{36}$}Also at DAMTP, University of Cambridge, Cambridge, United Kingdom\\
{$^{37}$}Also at The Cockcroft Institute, Daresbury, United Kingdom\\
{$^{38}$}Now at Diamond Light Source, Harwell, United Kingdom}
\end{flushleft}
\end{multicols}
}


==> figures/project/PowerContributions.tex <==
\begin{tikzpicture}[font=\sffamily,lines/.style={draw=none},scale=1,align=left]
\sansmath
\pie [%rotate = 90,
text = legend,
radius = 4.5,
sum=auto,
every only number node/.style={text=white},
style={lines},
pos={0,0},
    color={
    blue!60, %1
    cyan!60, %2
    yellow!60, %3
    orange!60, %4
    red!60, %5
    blue!60!cyan!60, %6
    cyan!60!yellow!60, %7
    red!60!cyan!60, %8
    red!60!blue!60, %9
    orange!60!cyan!60 %10
    },
] {
1/  Main beam injectors,
1 /  Main beam damping rings,
1 /  Main beam booster and transport,
1 /  Drive beam injectors,
1 /  Drive beam frequency multiplication and transport,
1 /  Two-beam acceleration,
1 /  Main linacs (klystron),
1 /  Interaction region,
1 /  Infrastructure and services,
1 /  Controls and operations
}

\pie [rotate = 90,
radius = 4.5,
sum=auto,
every only number node/.style={text=white},
style={lines},
    color={
    blue!60, %1
    cyan!60, %2
    yellow!60, %3
    orange!60, %4
    red!60, %5
    blue!60!cyan!60, %6
%    cyan!60!yellow!60, %7
    red!60!cyan!60, %8
    red!60!blue!60, %9
    orange!60!cyan!60 %10
    }
] {
6/  ,%/ Main beam injectors,
53/ ,%/ Main beam damping rings,
9/ ,%/ Main beam booster and transport,
45/ ,%/ Drive beam injectors,
14/ ,%/ Drive beam frequency multiplication and transport,
3/ ,%/ Two-beam acceleration,
4/ ,%/ Interaction region,
33/ ,%/ Infrastructure and services,
1/ %/ Controls and operations
}
\pie [rotate = 90,
radius = 4.5,
sum=auto,
every only number node/.style={text=white},
style={lines},
pos={18,0},
    color={
    blue!60, %1
    cyan!60, %2
    yellow!60, %3
%    orange!60, %4
%    red!60, %5
%    blue!60!cyan!60, %6
    cyan!60!yellow!60, %7
    red!60!cyan!60, %8
    red!60!blue!60, %9
    orange!60!cyan!60 %10
    }
] {
6 /,% Main beam Injectors,t
41 /,% Main beam damping rings,
8 / ,%Main beam booster and transport,
75 /,% Main linacs,
4 / ,%Interaction region,
29 / ,%Infrastructure and services,
1 / %Controls and operations
}
\node at (18,5) {\Large Klystron based option: 164\,MW};
\node at (0,5) {\Large Drive beam option: 168\,MW};
\end{tikzpicture}

